Gossip Learning with Linear Models on Fully Distributed Data

Machine learning over fully distributed data poses an important problem in peer-to-peer (P2P) applications. In this model we have one data record at each network node, but without the possibility to move raw data due to privacy considerations. For example, user profiles, ratings, history, or sensor readings can represent this case. This problem is difficult, because there is no possibility to learn local models, the system model offers almost no guarantees for reliability, yet the communication cost needs to be kept low. Here we propose gossip learning, a generic approach that is based on multiple models taking random walks over the network in parallel, while applying an online learning algorithm to improve themselves, and getting combined via ensemble learning methods. We present an instantiation of this approach for the case of classification with linear models. Our main contribution is an ensemble learning method which---through the continuous combination of the models in the network---implements a virtual weighted voting mechanism over an exponential number of models at practically no extra cost as compared to independent random walks. We prove the convergence of the method theoretically, and perform extensive experiments on benchmark datasets. Our experimental analysis demonstrates the performance and robustness of the proposed approach.

==> PerceptronConv.tex <==
\section{Perceptron convergence}

\begin{theorem} [Perceptron convergence]
\label{theorem:percconv}
\end{theorem}

\begin{proof}
\begin{equation}
\label{eq:percLB}
\begin{split}
	\left\langle w_{t+1},w_{opt}\right\rangle& = \left\langle w_{t} + \eta y_{t}x_{t},w_{opt}\right\rangle \\
	& = \left\langle w_{t},w_{opt}\right\rangle + \eta y_{t}x_{t}w_{opt} \\
	& \geq \left\langle w_{t},w_{opt}\right\rangle + \eta \alpha \\
	& \geq t\eta \alpha
\end{split}
\end{equation}

\begin{equation}
\label{eq:percUB}
\begin{split}
	\left\|w_{t+1}\right\|^2 &= \left\langle w_{t+1},w_{t+1}\right\rangle \\
	& = \left\langle w_{t} + \eta y_{t}x_t,w_{t} + \eta y_{t}x_t \right\rangle \\
	& = \left\|w_{t}\right\|^2 + \eta^2 y_{t}^2\left\| x_{t}\right\| ^2 + 2\eta y_{t}x_{t}w_{t} \\
	& \leq \left\|w_{t}\right\|^2 + \eta^2 y_{t}^2\left\| x_{t}\right\| ^2\\
	& \leq \left\|w_{t}\right\|^2 + \eta^2 \beta\\
	& \leq t\eta^2 \beta
\end{split}
\end{equation}

\begin{equation}
\label{eq:perc}
\begin{split}
	t\eta \alpha &\leq \left\langle w_{t+1},w_{opt}\right\rangle \leq \left\|w_{t+1}\right\| \left\|w_{opt}\right\| \leq \sqrt{t\eta^2 \beta}\left\|w_{opt}\right\|\\
	t^2\eta^2 \alpha^2 &\leq t\eta^2 \beta \left\|w_{opt}\right\|^2\\
	t & \leq \frac{\beta \left\|w_{opt}\right\|^2}{\alpha^2}
\end{split}
\end{equation}
Since in optimal case in every iteration the number of seen samples is 1, after $t+1$ iterations the learner was learned on $t$ samples. So we need at least $t \leq \frac{\beta \left\|w_{opt}\right\|^2}{\alpha^2}$ samples to reach this boundary.
\end{proof}


\begin{theorem} [Averaged perceptron convergence]
\label{theorem:avgperceptconv}
Given $\left(x_1,y_1\right),\ldots,\left(x_n,y_n\right)$ labeled training 
samples with the following restrictions: 1.) every samples are ''badly classified`` by 
the Perceptron algorithm in each step i.e. $\forall t: y_t\left\langle w_t,x_t\right\rangle\leq0$
and 2.) the training samples are bounded i.e $\argmax_{x_n}\left\|x\right\|^2\leq\beta$ .

The required number of iterations that has to be processed by the algorithm while reach its
stationarity is bounded with the expression given in~\ref{eq:avgperc}, where $w_{opt}$ is an optimal
solution for the classification problem i.e. $\forall \left( x,y \right) : y\left\langle x,w_{opt} \right\rangle \geq \alpha$.
\end{theorem}

\begin{proof} [The proof of the lower boundary]
\begin{equation}
\label{eq:avgpercLB}
\begin{split}
	\left\langle w_{t+1},w_{opt}\right\rangle& = \left\langle \frac{w_{t}^i + w_{t}^j}{2} + \eta y_{t}x_{t},w_{opt}\right\rangle \\
	& = \left\langle\frac{w_{t}^i + w_{t}^j}{2},w_{opt}\right\rangle + \eta y_{t}x_{t}w_{opt} \\
	& \geq \left\langle\frac{w_{t}^i + w_{t}^j}{2},w_{opt}\right\rangle + \eta \alpha \\
	& \geq t\eta \alpha
\end{split}
\end{equation}
\end{proof}

\begin{proof} [The proof of the upper boundary]
\begin{equation}
\label{eq:avgpercUB}
\begin{split}
	\left\|w_{t+1}\right\|^2 &= \left\langle w_{t+1},w_{t+1}\right\rangle \\
	& = \left\langle \frac{w_{t}^i + w_{t}^j}{2} + \eta y_{t}x_t,\frac{w_{t}^i + w_{t}^j}{2} + \eta y_{t}x_t \right\rangle \\
	& = \left\langle \frac{w_{t}^i + \eta y_{t}x_t + w_{t}^j + \eta y_{t}x_t}{2},\frac{w_{t}^i + \eta y_{t}x_t + w_{t}^j + \eta y_{t}x_t}{2} \right\rangle \\
	& = \frac{\left(w_{t}^i + \eta y_{t}x_t + w_{t}^j + \eta y_{t}x_t\right)^2}{4} \\
	& = \frac{1}{4}\left( \left\langle w_{t}^i,w_{t}^i\right\rangle + \left\langle w_{t}^j,w_{t}^j\right\rangle + 2\left\langle w_{t}^i,w_{t}^j\right\rangle \right) \\
	& \quad + \frac{1}{4}\left(4\eta^2y_{t}^2\left\|x_{t}\right\|^2 + 4\eta y_{t}w_{t}^{i}x_{t} + 4\eta y_{t}w_{t}^{j}x_{t} \right)\\
	& \leq \frac{1}{4} \left( \left\|w_{t}^i\right\|^2 + \left\|w_{t}^i\right\|^2 + 2\left\|w_{t}^i\right\|\left\|w_{t}^j\right\|\right) \\
	& \quad + \frac{1}{4}\left(4\eta^2y_{t}^2\left\|x_{t}\right\|^2 + 4\eta y_{t}w_{t}^{i}x_{t} + 4\eta y_{t}w_{t}^{j}x_{t} \right)\\
	& \leq \left\|w_{t}\right\|^2 + \eta^2y_{t}^2\left\|x_{t}\right\|^2 \\
	& \leq \left\|w_{t}\right\|^2 + \eta^2\beta \\
	& \leq t\eta^2\beta,
\end{split}
\end{equation}
where $\left\|w_{t}\right\| = \max \left(\left\|w_{t}^{i}\right\|,\left\|w_{t}^{j}\right\| \right)$.
\end{proof}

\begin{proof} [The proof of the iteration number boundary]
\begin{equation}
\label{eq:avgperc}
\begin{split}
t\eta \alpha &\leq \left\langle w_{t+1},w_{opt}\right\rangle \leq \left\|w_{t+1}\right\|\left\|w_{opt}\right\| \leq \sqrt{t\eta^2\beta}\left\|w_{opt}\right\| \\
t\eta \alpha &\leq \sqrt{t\eta^2\beta}\left\|w_{opt}\right\| \\
t^2\eta^2\alpha^2 &\leq t\eta^2\beta\left\|w_{opt}\right\|^2 \\
t & \leq \frac{\beta\left\|w_{opt}\right\|^2}{\alpha^2}.
\end{split}
\end{equation}
Since in optimal case in every iteration the number of seen samples is multiplied by a 2 factor, after $t+1$ iterations the learner was learned on $2^{t}-1$ samples. So we need at least $t \leq \log\left( \frac{\beta \left\| w_{opt} \right\|^2}{\alpha^2} + 1\right)$ samples for this logarithmic boundary.
\end{proof}


==> convergence.tex <==
\def\baseNumber{2}

\newpage
\begin{theorem} [P2Pegasos convergence]\label{theroem:pegasosconv}
Let $\left(x_1,y_1\right),\ldots,\left(x_n,y_n\right)$ be a labeled training 
sequence with the following restrictions: 1.) the elements of the sequence are ''badly classified`` by 
the {\sc{P2Pegasos}} algorithm in each step i.e. $\forall 1\leq t: y_t\left\langle w_t,x_t\right\rangle<1$
and 2.) the training samples are bounded i.e. $x_{max}=\argmax_{x_n}\left\|x\right\|^2$ . 
Moreover we assume that the ``distributed environment'' in which the algorithm runs is perfect in sense of 
in each time moment $t+1$ the necessary number of $t$ aged model is available 
i.e. there is no message delay or other embarrassing phenomena.

The required number of steps that has to be done by the algorithm while reach its
stationarity is bounded with the expression given in~\ref{eq:pegasosbound}, where $w_{opt}$ is an optimal
solution for the classification problem i.e. $\forall \left(x,y\right): y\left\langle w_{opt},x\right\rangle\geq 1$.

\begin{equation}
\label{eq:pegasosbound}
\begin{split}
t_{max}\ &\leq\ \baseNumber^{6\left\|w_{opt}\right\|^2}\\
\text{subject to}\ &\ \max\left(\baseNumber^{\left\|x_{max}\right\|^2},\baseNumber\right)\leq t_{max}
\end{split}
\end{equation}
\end{theorem}

\begin{proof}

In the proof we use the known bounds on Harmonic number showed in~\ref{eq:harmonic} and 
the Cauchy--Bunyakovsky--Schwarz inequality presented in~\ref{eq:cbs}.

\begin{gather}
log(n) + \frac{1}{2} + \frac{1}{2n} \leq H(n)=\sum_{i=1}^n\frac{1}{n} \leq log(n) + 1\label{eq:harmonic}\\
\left\langle x,y\right\rangle^2\leq \left\|x\right\|^2\left\|y\right\|^2\label{eq:cbs}
\end{gather}

%---------- Begin of Lower bound proof of P2Pegasos ----------
\emph{(Lower bound on the norm of the models)}
\begin{equation}
\label{eq:pegasos_lower_derivation}
\begin{split}
\left\langle w_{opt},w_{t+1}\right\rangle\ &=\ \left\langle w_{opt},\left(1-\frac{1}{t}\right)w_t + \frac{1}{\lambda t}y_t x_t\right\rangle \\
&=\ \left(1-\frac{1}{t}\right)\left\langle w_{opt},w_t\right\rangle + \frac{1}{\lambda t}\underbrace{y_t\left\langle w_{opt},x_t\right\rangle}_{\geq 1}\\
&\geq\ \left(1-\frac{1}{t}\right)\left\langle w_{opt},w_t\right\rangle + \frac{1}{\lambda t}\\
\end{split}
\end{equation}

Applying $t$ times the bound shown in~\ref{eq:pegasos_lower_derivation}, 
we got the lower bound presented in~\ref{eq:pegasos_lowerbound} assuming that a product in length 0 is equal to 1.

\begin{equation}
\label{eq:pegasos_lowerbound}
\begin{split}
\left\langle w_{opt},w_{t+1}\right\rangle\ &\geq\ \underbrace{\prod_{j=1}^t\left(1-\frac{1}{j}\right)\underbrace{\left\langle w_{opt},\underbrace{w_1}_{=\underline{0}}\right\rangle}_{=0}}_{=0} + \underbrace{\sum_{j=1}^t\underbrace{\prod_{k=j+1}^t\left(1-\frac{1}{k}\right)\frac{1}{\lambda j}}_{=\frac{1}{\lambda t}}}_{\geq \frac{1}{\lambda}\left(log(t) + \frac{1}{2} + \frac{1}{2t}\right)}\\
&\geq\ \frac{1}{\lambda}\left(log(t) + \frac{1}{2} + \frac{1}{2t}\right)\ \geq\ \frac{2tlog(t) + t + 1}{2t\lambda}\\
&\geq\ \frac{2tlog(t) + t}{2t\lambda}\ =\ \frac{2log(t) + 1}{2\lambda}\ \geq\ \frac{2log(t)}{2\lambda}\ =\ \frac{log(t)}{\lambda}\\
\left\|w_{opt}\right\|^2\left\|w_{t+1}\right\|^2\ &\geq\ \left\langle w_{opt},w_{t+1}\right\rangle^2\ \geq\ \frac{log^2(t)}{\lambda^2} \\
\left\|w_{t+1}\right\|^2\ &\geq\ \frac{log^2(t)}{\lambda^2\left\|w_{opt}\right\|^2}\\
\end{split}
\end{equation}

%The same bound presented in~\ref{eq:pegasos_lowerbound_samples} is hold in terms of the 
%number of processed samples ($n$), since the iteration counter ($t$) can be considered as 
%sample counter (the Pegasos algorithm processes one sample in each iteration).

%\begin{equation}
%\label{eq:pegasos_lowerbound_samples}
%\begin{split}
%\left\|w_{t+1}\right\|^2\ &\geq\ \frac{log^2(n)}{\lambda^2\left\|w_{opt}\right\|^2}\\
%\end{split}
%\end{equation}

%---------- Begin of Upper bound proof of P2Pegasos ----------
\emph{(Upper bound on the norm of the models)}
\begin{equation}
\label{eq:pegasos_upper_derivation}
\begin{split}
\left\|w_{t+1}\right\|^2\ &=\ \left\langle \left(1-\frac{1}{t}\right)w_t + \frac{1}{\lambda t}y_t x_t, \left(1-\frac{1}{t}\right)w_t + \frac{1}{\lambda t}y_t x_t \right\rangle \\
&=\ \underbrace{\left(1-\frac{1}{t}\right)^2}_{\leq 1} \left\|w_t\right\|^2 + 2\underbrace{\left(1-\frac{1}{t}\right)}_{\leq 1}\frac{1}{\lambda t}\underbrace{y_t\left\langle w_t,x_t\right\rangle}_{\leq 1} + \frac{1}{\lambda^2 t^2}\underbrace{y_t^2}_{= 1}\left\|x_t\right\|^2\\
&\leq\ \left\|w_t\right\|^2+2\frac{1}{\lambda t} + \frac{1}{\lambda^2 t^2}\left\|x_t\right\|^2 \\
\left\|w_{t+1}\right\|^2 - \left\|w_{t}\right\|^2\ &\leq\ \frac{2}{\lambda t} + \frac{1}{\lambda^2 t^2}\left\|x_t\right\|^2 \\
\end{split}
\end{equation}

Applying $t$ times the bound on the different of the norm of the models and 
summing up these bounds, 
we got the upper bound~\ref{eq:pegasos_upperbound} on the norm of $(t+1)$th model.

\begin{equation}
\label{eq:pegasos_upperbound}
\begin{split}
\left\|w_{t+1}\right\|^2\ &\leq\ \sum_{i=1}^{t}\frac{2}{\lambda i} + \frac{1}{\lambda^2 i^2}\ \cdot\ \underbrace{\left\|x_i\right\|^2}_{\leq \left\|x_{max}\right\|^2}\\
&\leq\ \frac{2}{\lambda}\underbrace{\sum_{i=1}^t\frac{1}{i}}_{\leq log(t)+1} + \frac{1}{\lambda^2}\left\|x_{max}\right\|^2\underbrace{\sum_{i=1}^t\frac{1}{i^2}}_{\leq 2}\\
&\leq\ 2\left(log(t)+1\right)\cdot\underbrace{\frac{1}{\lambda}}_{\leq\frac{1}{\lambda^2},\ \text{since}\ \lambda<1} + \frac{2}{\lambda^2}\left\|x_{max}\right\|^2\\
&\leq\ \frac{2\left(log(t)+1\right) + 2\left\|x_{max}\right\|^2}{\lambda^2} \\
&\leq\ \frac{2\left(log(t) + \left\|x_{max}\right\|^2 + 1\right)}{\lambda^2} \\
&\leq\ \frac{6log(t)}{\lambda^2} \\
\text{subject to}\ &\ \left\|x_{max}\right\|^2\leq log(t)\text{ and }1\leq log(t)\\
\text{i.e.}\ &\ \max\left(\baseNumber^{\left\|x_{max}\right\|^2},\baseNumber\right)\leq t\\
\end{split}
\end{equation}

%Again we can observe the same bound on number of required samples ($n$), since here the iteration 
%counter ($t$) can be considered as sample counter as above in case of lower bound. 
%The corresponding bound can be seen in~\ref{eq:pegasos_upperbound_samples}.

%\begin{equation}
%\label{eq:pegasos_upperbound_samples}
%\begin{split}
%\left\|w_{t+1}\right\|^2\ &\leq\ \frac{6log(n)}{\lambda^2} \\
%\text{subject to}\ &\ \max\left(\baseNumber^{\left\|x_{max}\right\|^2},\baseNumber\right)\leq n
%\end{split}
%\end{equation}
%---------- End of Upper bound proof of P2PegasosAvg convergence ----------

The stationarity is reached where the upper and lower bounds meets i.e. there can be existed an iteration 
number $t_{max}$ where the two bounds is satisfied by equality. The derived bound can be 
seen in~\ref{eq:pegasosbound_derivation}.

\begin{equation}
\label{eq:pegasosbound_derivation}
\begin{split}
\frac{log^2(t_{max})}{\lambda^2\left\|w_{opt}\right\|^2}\ &\leq\ \frac{6log(t_{max})}{\lambda^2}\\
log(t_{max})\ &\leq\ 6\left\|w_{opt}\right\|^2\\
t_{max}\ &\leq\ \baseNumber^{6\left\|w_{opt}\right\|^2}\\
\text{subject to}\ &\ \max\left(\baseNumber^{\left\|x_{max}\right\|^2},\baseNumber\right)\leq t_{max}
\end{split}
\end{equation}

\end{proof}
%---------- End of proof of P2Pegasos convergence ----------


Now let us discuss the {\sc{P2PegasosAvg}} algorithm which is a simple modification of the {\sc{P2Pegasos}} algorithm based
the following gradient update rule: 
$w_{t+1}=\left(1-\frac{1}{t}\right)\frac{w_{t}^{\left(i\right)}+w_{t}^{\left(j\right)}}{2} + \frac{1}{\lambda t}y_t x_t$. 
Here the top right index refer to the number of samples processed by the model and the bottom right one is the
iteration counter. Easy to see that --- it will be important in the following proof --- a model $w_{t+1}$ with age $t+1$
processed $2^{t}-1$ training samples assuming perfect ``distributed environment'' since this model spans a complete, $t+1$ depth
binary tree where each node add one samples to the model except the leaf ones which add zeros; and the number of the inner nodes in this tree is
equal to $2^{t}-1$.  

\newpage
\begin{theorem} [P2PegasosAvg convergence]\label{theroem:pegasosavgconv}
Let $\left(x_1,y_1\right),\ldots,\left(x_n,y_n\right)$ be a labeled training 
sequence with the following restrictions: 1.) the elements of the sequence are ''badly classified`` by 
the {\sc{P2PegasosAvg}} algorithm in each step i.e. $\forall 1\leq t: y_t\left\langle w_t,x_t\right\rangle<1$
and 2.) the training samples are bounded i.e. $x_{max}=\argmax_{x_n}\left\|x\right\|^2$ . 
Moreover we assume that the ``distributed environment'' in which the algorithm runs is perfect in sense of 
in each time moment $t+1$ the necessary number of $t$ aged model is available 
i.e. there is no message delay or other embarrassing phenomena.

%The required number of samples that has to be processed by the algorithm while reach its
%stationarity is bounded with the expression given in~\ref{eq:pegasosavgbound}, where $w_{opt}$ is an optimal
%solution for the classification problem i.e. $\forall \left(x,y\right): y\left\langle w_{opt},x\right\rangle\geq 1$.
The required number of steps that has to be done by the algorithm while reach its
stationarity is bounded with the expression given in~\ref{eq:pegasosbound}, where $w_{opt}$ is an optimal
solution for the classification problem i.e. $\forall \left(x,y\right): y\left\langle w_{opt},x\right\rangle\geq 1$.

\begin{equation}
\label{eq:pegasosavgbound}
\begin{split}
t_{max}\ &\leq\ \baseNumber^{6\left\|w_{opt}\right\|^2}\\
\text{subject to}\ &\ \max\left(\baseNumber^{\left\|x_{max}\right\|^2},\baseNumber\right)\leq t_{max}
\end{split}
\end{equation}
\end{theorem}

\begin{proof}

%---------- Begin of Lower bound proof of P2PegasosAvg ----------
\emph{(Lower bound on the norm of the models)}
\begin{equation}
\label{eq:pegasosavg_lower_derivation}
\begin{split}
\left\langle w_{opt},w_{t+1}\right\rangle\ &=\ \left\langle w_{opt},\left(1-\frac{1}{t}\right)\frac{w_t^{\left(i\right)}+w_t^{\left(j\right)}}{2} + \frac{1}{\lambda t}y_t x_t\right\rangle \\
&=\ \left(1-\frac{1}{t}\right)\frac{1}{2}\left\langle w_{opt},w_t^{\left(i\right)}+w_t^{\left(j\right)}\right\rangle + \frac{1}{\lambda t}\underbrace{y_t\left\langle w_{opt},x_t\right\rangle}_{\geq 1}\\
&\geq\ \left(1-\frac{1}{t}\right)\frac{1}{2}\left[\left\langle w_{opt},w_t^{\left(i\right)}\right\rangle+\left\langle w_{opt},w_t^{\left(j\right)}\right\rangle\right] + \frac{1}{\lambda t}\\
\end{split}
\end{equation}

Applying $t$ times the bound shown in~\ref{eq:pegasosavg_lower_derivation}, 
we got the lower bound presented in~\ref{eq:pegasosavg_lowerbound} assuming that a product in length 0 is equal to 1.

\begin{equation}
\label{eq:pegasosavg_lowerbound}
\begin{split}
\left\langle w_{opt},w_{t+1}\right\rangle\ &\geq\ \underbrace{\sum_{q=1}^{2^t}\frac{1}{2^t}\prod_{j=1}^t\left(1-\frac{1}{j}\right)\underbrace{\left\langle w_{opt},\underbrace{w_1^{\left(1\right)}}_{=\underline{0}}\right\rangle}_{=0}}_{=0} + \underbrace{\sum_{j=1}^t\underbrace{\prod_{k=j+1}^t\left(1-\frac{1}{k}\right)\frac{1}{\lambda j}}_{=\frac{1}{\lambda t}}}_{\geq \frac{1}{\lambda}\left(log(t) + \frac{1}{2} + \frac{1}{2t}\right)}\\
&\geq\ \frac{1}{\lambda}\left(log(t) + \frac{1}{2} + \frac{1}{2t}\right)\ \geq\ \frac{2tlog(t) + t + 1}{2t\lambda}\\
&\geq\ \frac{2tlog(t) + t}{2t\lambda}\ =\ \frac{2log(t) + 1}{2\lambda}\ \geq\ \frac{2log(t)}{2\lambda}\ =\ \frac{log(t)}{\lambda}\\
\left\|w_{opt}\right\|^2\left\|w_{t+1}\right\|^2\ &\geq\ \left\langle w_{opt},w_{t+1}\right\rangle^2\ \geq\ \frac{log^2(t)}{\lambda^2} \\
\left\|w_{t+1}\right\|^2\ &\geq\ \frac{log^2(t)}{\lambda^2\left\|w_{opt}\right\|^2}\\
\end{split}
\end{equation}

%The same bound presented in~\ref{eq:pegasosavg_lowerbound_samples} is hold in terms of the 
%number of processed samples ($n$), since the iteration counter ($t$) can be considered as 
%sample counter (the Pegasos algorithm processes one sample in each iteration).

%\begin{equation}
%\label{eq:pegasosavg_lowerbound_samples}
%\begin{split}
%\left\|w_{t+1}\right\|^2\ &\geq\ \frac{log^2(n)}{\lambda^2\left\|w_{opt}\right\|^2}\\
%\end{split}
%\end{equation}

%---------- Begin of Upper bound proof of P2PegasosAvg ----------
\emph{(Upper bound on the norm of the models)}

Let $w_{t,max}=\argmax_{i}\left\|w_{t}^{\left(i\right)}\right\|^2$ be introduced.

\begin{equation}
\label{eq:pegasosavg_upper_derivation}
\begin{split}
\left\|w_{t+1}\right\|^2\ &\leq\ \left\|w_{t+1,max}\right\|^2\\
&=\ \left\langle \left(1-\frac{1}{t}\right)\frac{w_t^{\left(i\right)} + w_t^{\left(j\right)}}{2} + \frac{1}{\lambda t}y_t x_t, \left(1-\frac{1}{t}\right)\frac{w_t^{\left(i\right)} + w_t^{\left(j\right)}}{2} + \frac{1}{\lambda t}y_t x_t \right\rangle\\
&=\ \frac{1}{4}\underbrace{\left(1-\frac{1}{t}\right)^2}_{\leq 1}\left\langle w_t^{\left(i\right)}+w_t^{\left(j\right)},w_t^{\left(i\right)}+w_t^{\left(j\right)}\right\rangle + \\
&\quad+2\underbrace{\left(1-\frac{1}{t}\right)}_{\leq 1}\frac{1}{\lambda t}y_t\frac{1}{2}\left\langle w_t^{\left(i\right)}+w_t^{\left(j\right)},x_t\right\rangle + \frac{1}{\lambda^2 t^2}\underbrace{y_t^2}_{= 1}\left\|x_t\right\|^2 \\
&\leq\ \frac{1}{4}\left(\underbrace{\left\|w_t^{\left(i\right)}\right\|^2+2\underbrace{\left\langle w_t^{\left(i\right)},w_t^{\left(j\right)}\right\rangle}_{\leq \left\|w_t^{\left(i\right)}\right\|\left\|w_t^{\left(j\right)}\right\|}+\left\|w_t^{\left(j\right)}\right\|^2}_{\leq 4\left\|w_{t,max}\right\|^2}\right) + \\
&\quad+\frac{1}{\lambda t}\left(\underbrace{y_t\left\langle w_t^{\left(i\right)},x_t\right\rangle}_{\leq 1} + \underbrace{y_t\left\langle w_t^{\left(j\right)},x_t\right\rangle}_{\leq 1}\right) + \frac{1}{\lambda^2 t^2}\left\|x_t\right\|^2\\
&\leq\ \left\|w_{t,max}\right\|^2 + \frac{2}{\lambda t} + \frac{1}{\lambda^2 t^2}\left\|x_t\right\|^2\\
%
\left\|w_{t+1,max}\right\|^2 - \left\|w_{t,max}\right\|^2\ &\leq\ \frac{2}{\lambda t} + \frac{1}{\lambda^2 t^2}\left\|x_t\right\|^2 \\
\end{split}
\end{equation}

Applying $t$ times the bound on the different of the norm of the models and 
summing up these bounds, 
we got the upper bound~\ref{eq:pegasosavg_upperbound} on the norm of $(t+1)$th model.

\begin{equation}
\label{eq:pegasosavg_upperbound}
\begin{split}
\left\|w_{t+1}\right\|^2\ &\leq\ \left\|w_{t+1,max}\right\|^2\ \leq\ \sum_{i=1}^{t}\frac{2}{\lambda i} + \frac{1}{\lambda^2 i^2}\ \cdot\ \underbrace{\left\|x_i\right\|^2}_{\leq \left\|x_{max}\right\|^2}\\
&\leq\ \frac{2}{\lambda}\underbrace{\sum_{i=1}^t\frac{1}{i}}_{\leq log(t)+1} + \frac{1}{\lambda^2}\left\|x_{max}\right\|^2\underbrace{\sum_{i=1}^t\frac{1}{i^2}}_{\leq 2}\\
&\leq\ 2\left(log(t)+1\right)\cdot\underbrace{\frac{1}{\lambda}}_{\leq\frac{1}{\lambda^2},\ \text{since}\ \lambda<1} + \frac{2}{\lambda^2}\left\|x_{max}\right\|^2\\
&\leq\ \frac{2\left(log(t)+1\right) + 2\left\|x_{max}\right\|^2}{\lambda^2} \\
&\leq\ \frac{2\left(log(t) + \left\|x_{max}\right\|^2 + 1\right)}{\lambda^2} \\
&\leq\ \frac{6log(t)}{\lambda^2} \\
\text{subject to}\ &\ \left\|x_{max}\right\|^2\leq log(t)\text{ and }1\leq log(t)\\
\text{i.e.}\ &\ \max\left(\baseNumber^{\left\|x_{max}\right\|^2},\baseNumber\right)\leq t\\
\end{split}
\end{equation}

%Again we can observe the same bound on number of required samples ($n$), since here the iteration 
%counter ($t$) can be considered as sample counter as above in case of lower bound. 
%The corresponding bound can be seen in~\ref{eq:pegasosavg_upperbound_samples}.

%\begin{equation}
%\label{eq:pegasosavg_upperbound_samples}
%\begin{split}
%\left\|w_{t+1}\right\|^2\ &\leq\ \frac{6log(n)}{\lambda^2} \\
%\text{subject to}\ &\ \max\left(\baseNumber^{\left\|x_{max}\right\|^2},\baseNumber\right)\leq n
%\end{split}
%\end{equation}
%---------- End of Upper bound proof of P2PegasosAvg convergence ----------

The stationarity is reached where the upper and lower bounds meets i.e. there can be existed an iteration 
number $t_{max}$ where the two bounds is satisfied by equality. The derived bound can be 
seen in~\ref{eq:pegasosbound_derivation}.

\begin{equation}
\label{eq:pegasosbound_derivation}
\begin{split}
\frac{log^2(t_{max})}{\lambda^2\left\|w_{opt}\right\|^2}\ &\leq\ \frac{6log(t_{max})}{\lambda^2}\\
log(t_{max})\ &\leq\ 6\left\|w_{opt}\right\|^2\\
t_{max}\ &\leq\ \baseNumber^{6\left\|w_{opt}\right\|^2}\\
\text{subject to}\ &\ \max\left(\baseNumber^{\left\|x_{max}\right\|^2},\baseNumber\right)\leq t_{max}
\end{split}
\end{equation}

%---------- End of proof of P2PegasosAvg convergence ----------
\end{proof}

